Asymptotic distribution of the Markowitz portfolio

The asymptotic distribution of the Markowitz portfolio is derived, for the general case (assuming fourth moments of returns exist), and for the case of multivariate normal returns. The derivation allows for inference which is robust to heteroskedasticity and autocorrelation of moments up to order four. As a side effect, one can estimate the proportion of error in the Markowitz portfolio due to mis-estimation of the covariance matrix. A likelihood ratio test is given which generalizes Dempster's Covariance Selection test to allow inference on linear combinations of the precision matrix and the Markowitz portfolio. Extensions of the main method to deal with hedged portfolios, conditional heteroskedasticity, conditional expectation, and constrained estimation are given. It is shown that the Hotelling-Lawley statistic generalizes the (squared) Sharpe ratio under the conditional expectation model. Asymptotic distributions of all four of the common `MGLH' statistics are found, assuming random covariates. Examples are given demonstrating the possible uses of these results.

==> Makefile <==

######################
######################
# makefile generated 
# dude makefile 
# created by s.e.pav 
# $Id: Makefile 89 2006-01-26 20:59:08Z spav $
######################
######################

############### FLAGS ###############

# these don't work at times
# in that case set these by hand?

LATEX       := $(shell which latex)
BIBTEX      := $(shell which bibtex)
PDFLATEX    := $(shell which pdflatex)
MAKEINDEX   := $(shell which makeindex)
PAGER   		:= $(shell which less)
ASPELL  		:= $(shell which aspell)

RLIB         = /usr/lib64/R

#TEXINPADD    = .:$(HOME)/sys/etc/tex:$(HOME)/sys/etc/tex/SEPtex:$(HOME)/work/math/TEX:$(RLIB)/share/texmf/tex/latex
TEXINPADD    = .:$(RLIB)/share/texmf/tex/latex

PRETEX       = TEXINPUTS=$(TEXINPADD):$$TEXINPUTS
PREBIB       = BSTINPUTS=$(TEXINPADD):$$BSTINPUTS \
               BIBINPUTS=$(TEXINPADD):$$BIBINPUTS 

PREIDX       = INDEXSTYLE=$(TEXINPADD):$$INDEXSTYLE

#undoes psfrag for pdf
UNPSFRAG		 = perl $(HOME)/sys/bin/unpsfrag.pl
#unroll commands
DETEXIFY		 = perl $(HOME)/sys/perl/detexify.pl

SCREEN_SIZE  = normal
# include	$(HOME)/sys/etc/.Makefile.local

PROJECT      = asymarko
TEX_SOURCE   = $(PROJECT).tex
BIB_SOURCE   = $(PROJECT).bib
DVI_TARGET   = $(PROJECT).dvi
PDF_TARGET   = $(PROJECT).pdf
BBLS         = $(PROJECT).bbl

TAR 				?= $(shell which tar)

#SAVE
# tracked projects
PROJECTS     = $(PROJECT) 
#UNSAVE
# add on dependencies (subchapters of asymarko)
#R_DEPS 			 = defs.R
#TEX_EXTRAS   = sharpe_shortcuts.tex mac_overfit.tex skew_study_show.tex
#TEX_EXTRAS  += $(R_DEPS)
R_DEPS 			 = 
TEX_EXTRAS   = SharpeR.sty SharpeR.bib
# nonlocal dependencies
STY_FILES    = 

#aspell
ASPELL_FLAGS = 

#dot
DOT_FLAGS    = 

SHOW_PNG     = $(wildcard dude_show*.png)
SHOW_EPS     = $(patsubst %.png,%.eps,$(SHOW_PNG))


############## DEFAULT ##############

default : all

############## MARKERS ##############

.PHONY   : 
.SUFFIXES: .tex .bib .dvi .ps .pdf .eps
.PRECIOUS: %.dvi %.ps %.pdf %.jpg %.gif %.eps

############ BUILD RULES ############

.PHONY   : help 

# this will have to change b/c of inclusion file names...
help:  ## generate this help message
	@grep -h -P '^(([^\s]+\s+)*([^\s]+))\s*:.*?##\s*.*$$' $(MAKEFILE_LIST) | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-30s\033[0m %s\n", $$1, $$2}'


## the old way using Sweave
#%.tex : %.Rnw $(R_DEPS)
		#R CMD Sweave $<


%.tex : %.Rnw $(R_DEPS)
		Rscript -e 'require(knitr);knit("$<")'
		@-perl -pi -e 's/(syn|ft)=(Rnw|rnoweb)/$$1=tex/g;' $@

%.R : %.Rnw
		Rscript -e 'require(knitr);knit("$<",tangle=TRUE)'
		@-perl -pi -e 's/(syn|ft)=(Rnw|rnoweb)/$$1=R/g;' $@

%.pdf : %.tex
	latexmk -f -bibtex -pdf -pdflatex="$(PDFLATEX)" -use-make $<

%.dep.dot : %.tex %.dvi $(STY_FILES)
		echo digraph G \{ > $@;
		$(PRETEX) $(LATEX) $< | grep 'DEP:' | perl -pe 's/DEP://;s/\\hbox {}//g;' >> $@
		echo \} >> $@;

%.ps : %.dvi
		dvips $(DVIPS_FLAGS) -o $@ $< 

#%.pdf : %.dvi
		#dvips $(DVIPDF_FLAGS) -o $*.ps $< 
		#ps2pdf $*.ps
		#-rm -f $*.ps

# converting to pdf the hard way

%.pdftex : %.tex
		$(UNPSFRAG) $<
		cp _$< $@

%.pdf : %.pdftex
		$(PDFLATEX) $<

%.mergepdf :
		gs -dBATCH -dNOPAUSE -q -sDEVICE=pdfwrite -sOutputFile=$@ $(*)*.pdf

# roll commands from sty files

%.detex : %.tex
		@-if ! [ -r $@ ]; then cp $< $@; fi
		$(DETEXIFY) $@ >> $@;

# crappy ps from pdf.
%.craps : %.pdf
		a2ps -X'ascii' -M'Letter' -R --columns=1 -o $*.ps $<

# crappy ps from edp
%.craps : %.edp
		a2ps -X'ascii' -M'Letter' -R --columns=2 -o $*.ps $<

# reverse?
%.pdf : %.eps
		epstopdf $<

# crappy ascii anyone?
%.txt : %.ps
		ps2ascii $< > $@

# crappy html anyone?
%.html : %.tex
		$(HTLATEX) $< 
		-rm -f tex4ht.fls $*.4ct $*.4tc $*.lg $*.idv $*.xref $*.tmp

# tex extras
%.bbl : %.bib
		$(PREBIB) $(BIBTEX) $*

%.bbl : %.aux
		$(PREBIB) $(BIBTEX) $*

%.ind : %.idx
		$(PREIDX) $(MAKEINDEX) $*

# convert from xfig
%.eps : %.fig
		/bin/rm -f $@ 
		fig2dev -L ps $< > $@

# see http://electron.mit.edu/~gsteele/pdf/ 
%.eps : %.png
		convert $< $@

# make a graph
%.dot : %.flc
		perl $(HOME)/sys/perl/flowcharter.pl $< > $@

%.ps : %.dot
		dot $(DOT_FLAGS) -Tps $< -o $@

%.fig : %.dot
		dot $(DOT_FLAGS) -Tfig $< -o $@

# viewing targets
#$(DVIVIEWER) $(XDVI_FLAGS) $*.dvi
%.xsee : %.dvi
		$(DVIVIEWER) $(EVINCE_DVI_FLAGS) $*.dvi
		
%.pdfsee : %.pdf
		$(PDF_VIEWER) $(PDFSEE_FLAGS) $*.pdf

# check a document
%.chk : %.dup %.spell

# check spelling
%.spell : %.tex
		$(ASPELL) $(ASPELL_FLAGS) --dont-tex-check-comments -t -l < $< | sort | uniq | $(PAGER)

# check duplicate words
%.dup : %.tex
		perl -an -F/\\s+/ -e 'BEGIN { $$last = q[]; $$line = 0; $$prevline = q[];}\
		$$line++;$$first = 1;\
		foreach $$word (@F) {\
		if ($$word eq $$last) {\
		if ($$first) { print qq[duplicate $$word, lines ],($$line-1),qq[-$$line:\n$$prevline$$_]; }\
		else { print qq[duplicate $$word, line $$line:\n$$_]; } }\
		$$last = $$word; $$first = 0; } \
		$$prevline = $$_;' < $< | $(PAGER)

# put into a tar file
%.tar : %.manif
		@ $(TAR) -chvf $@ -T $< $< Makefile

%.tgz : %.manif
		@ $(TAR) -chzvf $@ -T $< $< Makefile


############# CLEAN UP ##############

# clean up
%.clean : 
		-rm -f $*.aux $*.log $*.dvi $*.bbl $*.blg $*.toc $*.ilg $*.ind
		-rm -f $*.out $*.idx $*.lot $*.lof $*.brf $*.nav $*.snm
%.realclean : %.clean
		-rm -f $*.ps $*.pdf
		-rm -f $*-[0-9][0-9][0-9]*.eps $*-[0-9][0-9][0-9]*.pdf


############### RULES ###############

# an easy target
# all: $(DVI_TARGET) $(BBLS) figure/Curve_fitting.eps 
all: $(DVI_TARGET) $(BBLS) 

ratarb: ratarb.dvi $(BBLS)

release.tex: $(PROJECT).tex
	perl -pe 's{figure/}{};' < $< > $@

release : release.tex
	mv release.tex $(PROJECT).tex
	@-echo "upload to arxiv"

dvis: $(patsubst %,%.dvi,$(PROJECTS))
pss: $(patsubst %,%.ps,$(PROJECTS))
pdfs: $(patsubst %,%.pdf,$(PROJECTS))

# targets
$(DVI_TARGET): $(TEX_SOURCE) $(TEX_EXTRAS) $(STY_FILES)
#$(PDF_TARGET): $(PS_TARGET)
$(PDF_TARGET): $(TEX_SOURCE) $(TEX_EXTRAS)

hints :
	@-grep slides Makefile
	@-grep today Makefile

# see them 
presee: $(PROJECT).xsee
xsee: $(PROJECT).xsee
see: $(PROJECT).psee
pdfsee: $(PROJECT).pdfsee

# check it

spell: $(PROJECT).spell 

# clean up
clean: $(patsubst %,%.clean,$(PROJECTS))
realclean: $(patsubst %,%.realclean,$(PROJECTS))
		-rm -f Rplots.pdf

cleancache: 
		echo "killing knitr cache! ack!"
		-rm -rf cache

superclean: realclean cleancache

safe: realclean
		@$(TAR) -cvf $(TAR_FILE) $(TAR_MAJORS) $(SUB_FIGS)
		@ -$(TAR) -uvf $(TAR_FILE) $(DVI_TARGET)
		@ -$(TAR) -uvf $(TAR_FILE) $(TAR_MINORS) 
		@ -$(TAR) -tvf $(TAR_FILE)
		rm -f $(TARBZ_FILE)
		bzip2 $(TAR_FILE)

# see http://www.latex-community.org/forum/viewtopic.php?f=5&t=2070 
# sigh
show_extras: $(SHOW_EPS)

.tags :
	nice -n 18 ctags -f .tmp_tags --recurse --language-force=R --fields=+i `find . -regextype posix-egrep -regex '.*.R(nw)?'`;
	mv .tmp_tags $@

############# ONE OFFS ##############

figure/Curve_fitting.jpg :
	#wget -O $@ "http://www.automatedtrader.net/Files/images/Mags/Issue_04_Jan_07/Strategies/Curve%20fitting.jpg"
	wget -O $@ "www.imgur.com/5oOkkSR.jpg"

figure/Curve_fitting.eps : figure/Curve_fitting.jpg
	convert $^ $@

######################
######################

######################
######################
# remake the makefile from the stub directory
makefile:
		cp Makefile .oldMakefile;
		perl -pe 's/\s+PROJ_NAME/ $(PROJECT)/;s{\s+CWD_NAME}{ $(DIR_STUB)};' < $(STUB)/Makefile > Makefile;
		-diff Makefile .oldMakefile;
		-rm -i .oldMakefile;

#for vim modeline: (do not edit)
# vim:ts=2:sw=2:tw=79:fdm=marker:fmr=FOLDUP,UNFOLD:cms=#%s:tags=tags;:syn=make:ft=make:ai:si:cin:nu:fo=croqt:cino=p0t0c5(0:

